Recognisable languages over monads

The principle behind algebraic language theory for various kinds of structures, such as words or trees, is to use a compositional function from the structures into a finite set. To talk about compositionality, one needs some way of composing structures into bigger structures. It so happens that category theory has an abstract concept for this, namely a monad. The goal of this paper is to propose monads as a unifying framework for discussing existing algebras and designing new algebras.

==> intro.tex <==
\section{Introduction}
\begin{itemize}
	\item There are popular theorems in formal language theory, which have been stated and proved in multiple different settings, and which can be proved on the general level of monads. One example is the existence of syntactic algebras, also known as the Myhill-Nerode theorem. Another example is the Eilenberg Pseudovariety Theorem, which has been proved for: 
\end{itemize}






==> logical-structures.tex <==
\section{Logical structures in monads}
\label{sec:logical-structures-in-monads}

 We try to present an abstract definition of positions which specializes to the standard notion of positions in all cases studied in this paper. Let $\monad$ be a monad in the category of sets, let $\Sigma$ be a set, and let $w \in \monad \Sigma$. A \emph{coloring} of $w$  consists of a function $f : \Gamma \to \Sigma$ and an  element $v \in \monad \Gamma$ such that $\monad f (v) =w$.  A \emph{an indexing of $w$} is an element $v \in \monad \Gamma$ for some $\Gamma$, such that there is a unique 
  $w \in \monad \Sigma$ is a $w$-coloring $f : \Gamma \to \Sigma$ such that every $w$-coloring factors through $f$.
  The set $\Gamma$ in an indexing of $w$ can be viewed as the positions in $w$.  This works for all the monads described before, but there are monads well it will not work.
  \begin{center}
  	(TODO: counterexample of profinite monad)
  \end{center}
  
  
  \begin{center}
  	(TODO: complete)
  \end{center}
 %   For elements $x_1,\ldots,x_n$  We say that positions $x_1,\ldots,x_n \in \Gamma$ satisfy a predicate if $\monad t$
 %
 % maps $v$ to $w$.  A \emph{universe} of $w$ is a set $\Gamma$ such that
 % a  A \emph{pre-universe} for $w$ is a set $U$ and $v \in \monad U$ such that $w= \monad f (v)$ holds for some $f : U \to \Sigma$.


==> nominal.tex <==
\section{Nominal sets}
\newcommand{\nommonoid}{\mathsf M}
In this section, we present a monad in a category other than sets. Consider the category where objects are equivariant nominal sets, and the morphisms are equivariant functions. Let $\nommonoid$ be the monad of finite words in this category, i.e.~$\nommonoid X = X^*$.   Define an object to be finite if it is orbit-finite, and an $\nommonoid$-algebra to be finite if its universe is orbit-finite.

It is not difficult to see that finite $\nommonoid$-algebras are the same thing as (equivariant) nominal monoids as defined in~\cite{DBLP:journals/mst/Bojanczyk13}. We mention this monad because it fails two natural properties:
\begin{itemize}
	\item The language of all sequences of atoms is  $\nommonoid$-recognisable, but it does not contain any  $\nommonoid$-recognisable singletons. This is because of the equivariance.
	\item $\nommonoid$-recognisable languages are not closed under images of $\nommonoid$-morphisms. This is because the language ``some two atoms are different'' is not $\nommonoid$-recognisable, but it is an image of a $\nommonoid$-recognisable language.
\end{itemize}



==> pin.tex <==
\section{Two applications of profinite monads}
In this section we give two applications of profinite objects. The application result says that profinite objects	 can be used to describe lattices of languages, although the theorem is not effective in any way. The second application says that although the profinite object makes sense for any class of languages, e.g.~for decidable languages, only  recognisable languages can be used if one wants the algebraic structure of the monad to be consistent with the topology.






\subsection{Uniform continuity of term operations}
\label{sec:con-top-thm}

%
% \paragraph*{A combinatorial lemma.} To prove the second item  of Theorem~\ref{thm:consistent-topology}, we will use a simple combinatorial lemma about functions of two arguments.
% For a  function $f : X \times Y \to C$ define the \emph{left equivalence} to be the equivalence relation on $X$ which identifies $x,x' \in X$ if
% \begin{align*}
%  f(x,y)=f(x',y) \qquad \mbox{ for every $y \in Y$}.
% \end{align*}
% Likewise we define the right equivalence, an equivalence relation on $Y$. If $C$ is finite, the either both left and right equivalence relations have finite index, or both have infinite index.
%
% \begin{lemma}\label{lem:ramsey-like}
% 	Let $R \subseteq X \times Y$ be a such that left (equivalently, right) equivalence has infinite index. Then there are
% \begin{align*}
% 	x_1,x_2,\ldots \in X \qquad y_1,y_2,\ldots \in Y
% \end{align*}
% such that every $n < m \in \Nat$ satisfy
% \begin{align*}
% 	(x_n,y_n) \in R \qquad \mbox{iff} \qquad (x_n,y_m) \not \in R.
% \end{align*}
% \end{lemma}
% \begin{pr}
% 	In the proof, we  treat $R$ as its characteristic function.
% 	Choose $x_1 \in X$ to be such that $R(x_1,\_)$ is neither empty nor full. There must be some  $c_1 \in \set{0,1}$ such that
% 	\begin{align*}
% 		Y_1 = \set{y \in Y: R(x_1,y)=c_1}
% 	\end{align*}
% 	represents infinitely many classes of right equivalence.  Define $y_1$ to be some element of $Y$ such that $R(x_1,y_1) \neq c_1$. It is not difficult to check that $R$ restricted to
% 	\begin{align*}
% 		(X - \set{x_1}) \times Y_1
% 	\end{align*}
% 	has infinite index of right equivalence. Therefore, we can reapply the process, yielding a sequence of subsets
% 	\begin{align*}
% 		Y \supsetneq Y_1 \supsetneq Y_2 \supsetneq \cdots  \qquad
% 	\end{align*}
% 	and elements
% 	\begin{align*}
% 		x_n \in X \qquad y_n \in Y_{n-1}-Y_n \qquad c_n \in C
% 	\end{align*}
% 	such that for every $n<m$ we have
% 	\begin{align*}
% 		R(x_n,y_n) = c_n \qquad R(x_n,y_m) \neq c_n.
% 	\end{align*}
% 	By extracting a subsequence, we can assume that all $c_n$ are equal, which yields the lemma.
% \end{pr}
%
%
%
% \paragraph*{Proof of item 2 in Theorem~\ref{thm:consistent-topology}.} Consider some language $L \subseteq \alg$ that is not $\monad$-recognisable. By the Syntactic Morphism Theorem, the relation
% 	\begin{align*}
% 		\set{ (p,a) : \sem{p}(a) \in L} \subseteq   \upol 1 \alg \times \alg
% 	\end{align*}
% 	has infinite index of right equivalence
% 	 Because $P$ is assumed to be observationally complete, it follows that
% 	\begin{align*}
% 		\set{ (p,a) : \sem{p}(a) \in L} \subseteq   P \times \alg
% 	\end{align*}
% 	has infinite index of right equivalence as well. Applying Lemma~\ref{lem:ramsey-like}, we get some  $p_n \in P$ and $a_n \in A$ such that every $n< m \in \Nat$ satisfy
% 	\begin{align*}
% \sem{p_n}(a_n) \in L \qquad \mbox{iff} \qquad \sem{p_n}(a_m) \not \in L.
% 	\end{align*}
% 	Without loss of generality assume that $\sem{p_n}(a_n) \in L$ holds for all $n$.
% 	Because $P$ has a finite cover,  we can assume without loss of generality that there is  some $q \in \upol 1 \balg$ which covers every $p_n$. Because the monad is finitary, $q \in \monad (B_0 \sqcup \set 1)$ for some finite subset $B_0$ of the universe of $\balg$. In other words, for every $n$ there is some
% 	\begin{align*}
% 		h_n : B_0 \to A \qquad \mbox{with }p_n= h(q).
% 	\end{align*}
% For $n,m$ define
% 	\begin{align*}
% 		f_{nm} : (B_0 \sqcup \set 1) \to A
% 	\end{align*}
% 	to be the disjoint union of $h_n$ and the valuation that maps $1$ to $a_m$.
% 	 It follows that
% 	\begin{align*}
% 		\sem{p_n}(a_m) =  \sem{q}(f_{nm}).
% 	\end{align*}
% 	By extracting subsequnces, and using compactness of the topology,  we may assume that the sequence $(h_n)_n$ is Cauchy, and so is the sequence $(a_n)_n$. It follows that the sequence of valuations
% 	\begin{align*}
% 		f_{11},f_{12},f_{22},f_{23},\ldots,f_{nn},f_{n(n+1)},\ldots
% 	\end{align*}
% 	is Cauchy. However, applying $\sem{q}$ to this sequence yields a sequence that  alternates between $L$ and its complement, and is therefore not Cauchy.

==> rubbish.tex <==



\paragraph*{Topological structure.}
To prove~\eqref{eq:gh-diagram}, we  use a bit of  topology. 
% We see a finite $\monad$-algebra as a topological space equipped with the discrete topology, where every set is open and closed, or equivalently, equipped with a distance where the distance between every two different elements of the universe is $1$. We will use the distance to talk about uniform continuity.
We view $\monad \Sigma$ and  $\promonad \Sigma$, respectively, as topological spaces, with the base open sets being of the form $h^{-1}(a)$ and $\bar h ^{-1}(a)$, respectively, where $h : \monad \Sigma \to \alg$ is a $\monad$-morphism into a fintie $\monad$-algebra containing $a$.
%
%   $\promonad \Sigma$ as a topological space\footnote{Another view on $\promonad \Sigma$ is that it is homeomorphic to the Stone dual of the Boolean algebra of subsets of $\monad \Sigma$  recognised by $\monad$-morphisms into finite $\monad$-algebras.
% }, where the base open sets are sets of the form
% \begin{align*}
% 	\set{ w : \bar h(w) = a} \qquad \mbox{where }h : \monad \Sigma \to \alg \mbox{ and }a \in A.
% \end{align*}
 There is a natural function
\begin{align*}
	\xymatrix{\monad \Sigma \ar@{^{(}->}[r] & \promonad \Sigma}
\end{align*}
which maps $w$ to the morphism type $h \mapsto h(w)$.  The assumption that the monad is Hausdorff says that the above function is injective. The image of this injection is called \emph{real morphism types}.  It is easy to see that real morphism types are dense in all morphism types, i.e.~every base open set contains a real  morphism type.

The following lemma says that $\promonad \Sigma$ is the Cech-Stone compactification of $\monad \Sigma$.
\begin{lemma}\label{lem:cech-stone}
	Let $\Sigma$ be a set. For every continuous function $f  : \monad \Sigma \to X$ into a compact Hausdorff topological space there exists a unique continuous  $\bar f$ which extends $f$ in the sense that the following diagram commutes:
	\begin{align*}
		\xymatrix{ \monad \Sigma \ar@{^{(}->}[r] \ar[rd]_{f} & \promonad \Sigma \ar[d]^{\bar f} \\ & X}
	\end{align*}
\end{lemma}
\begin{pr}
	(TODO: find citation somewhere)	%
	% For  $w \in \promonad \Sigma$, consider the set
	% \begin{align*}
	% 	\bigcap_{X} \overline {f(X)}
	% \end{align*}
	% where $X$ ranges over closed subsets of $\monad \Sigma$ such that $\bar X \ni x$. We claim that the above set contains at most one element. Toward a contradiction, suppose that the above set contains two elements $x,y \in X$. Because $X$ is Hausdorff, there are disjoint open sets $U_x \ni x$ and $U_y \ni y$.  The inverse images
	% \begin{align*}
	% f^{-1}(U_x), f^{-1}(U_y) \subseteq \monad \Sigma
	% \end{align*}
	% are disjoint open sets.
	%
	%
	% Because $f$ is continuous, there are base open sets $V_x, V_y \ni $
\end{pr}

If $h : \monad \Sigma \to \alg$ is a $\monad$-morphism into a finite $\monad$-algebra, then $\bar h$ can be interpreted in two ways: as the function defined in~\eqref{eq:barh-definition}, or as the function defined in Lemma~\ref{lem:cech-stone}. One can check that the function defined in~\eqref{eq:barh-definition} is continuous and extends $h$, and therefore the two interpretations are the same.






******



% 	\begin{lemma}\label{lem:chasing-one}
% 		If $h : \alg \to \balg$ is a $\monad$-morphism of finite $\monad$-algebras, then the following diagram commutes
% 				\begin{align*}
% 					\vcenter{\xymatrix @R=1pc
% 						{ \promonad A \ar[d]_{ \overline{\mult_\alg}}  \ar[r]^{\promonad h} & \promonad B \ar[d]^{\overline{\mult_\balg}}\\
% 						 A \ar[r]^{h}  & B
% 						}}
% 				\end{align*}\
% 	\end{lemma}
% 	\begin{pr}
% \begin{eqnarray*}
% 	\overline{\mult_\balg} (\promonad h (w)) &= & \eqexplain{by definition of $\promonad h$}\\
% 	\overline{\mult_\balg \circ \monad h} (w) &= & \eqexplain{because $h$ is a $\monad$-morphism}\\
% 	\overline{h \circ \mult_\alg}(w)&=& \eqexplain{by definition of a $\monad$-morphism type}\\
% 	h (\overline{\mult_\alg}(w))
% \end{eqnarray*}
% 		By applying the diagram from Lemma~\ref{lem:cech-stone}  for the special case of the multiplication operations in $\alg$ and $\balg$, and using the assumption that  $h$ is a $\monad$-morphism, we see that the following diagram commutes
% 			\begin{align}\label{eq:tall-diagram}
% 				\vcenter{\xymatrix @R=2pc@C=3pc
% 					{ \monad A  \ar@{^{(}->}[d]  \ar[r]^{\monad h}& \monad B \ar@{^{(}->}[d]  \\   \promonad A \ar[d]_{\overline{\mult_\alg}} & \promonad B \ar[d]^{\overline{{\mult_\balg}}}\\
% A \ar[r]^{h}  & B
% 					}}
% 			\end{align}
% From the definition, one sees that $\promonad h$ extends $\monad h$ in the sense that the following diagram commutes
% 				\begin{align}\label{eq:promonad-extends}
% 					\vcenter{\xymatrix @R=1pc
% 					{ \monad A  \ar[r]^{\monad h} \ar@{^{(}->}[d] & \monad B \ar@{^{(}->}[d]  \\
% 					\promonad A \ar[r]_{\promonad h}&  \promonad B
% 					}}.
% 				\end{align}
% 				By combining~\eqref{eq:tall-diagram} and~\eqref{eq:promonad-extends}, we  see that the following diagram commutes
% 			\begin{align*}
% 				\vcenter{\xymatrix @R=2pc@C=3pc
% 					{ \monad A  \ar@{^{(}->}[d]   \\   \promonad A \ar[d]_{\overline{\mult_\alg}} \ar[r]^{\promonad h} & \promonad B \ar[d]^{\overline{{\mult_\balg}}}\\
% 					A \ar[r]^{h}  & B
% 					}}
% 			\end{align*}
% 			It is not difficult to check that $\promonad h$ is  continuous, and also $\overline{\mult_\alg}$ and $\overline{\mult_\balg}$ are continuous, assuming discrete topologies on the finite algebras.  The lower part of the diagram above describes two continuous functions from $\promonad A$ to the compact Haudorff space $\balg$, which extend
% 		 the continuous function
% 	 \begin{align*}
% 	h \circ  	\mult_\alg = \mult_\balg \circ \monad h.
% 	 \end{align*}
%  Therefore, by the uniqueness part of Lemma~\ref{lem:cech-stone}, the lower part of the diagram commutes.
%  \end{pr}
%
% 	\begin{lemma}\label{lem:chasing-two}
% If $\alg,\balg$ are finite $\monad$-algebras and  $h : \monad \Sigma \to \alg$ and $g : \alg \to \balg$ are $\monad$-morhpisms, then the following diagram commutes.
% 		\begin{align*}
% 			\xymatrix{ \promonad \Sigma \ar[r]^{\bar h} \ar[dr]_{\overline{g \circ h}}&  A \ar[d]^{ g}\\
% 			& B}
% 		\end{align*}
% 	\end{lemma}
% 	\begin{pr}
% 		It is easy to see that following diagram commutes:
% 				\begin{align*}
% 					\xymatrix{\monad \Sigma \ar@{^{(}->}[r] & \promonad \Sigma \ar[r]^{\bar h} \ar[dr]_{\overline{g \circ h}}&  A \ar[d]^{ g}\\
% 					&& B}
% 				\end{align*}
% 		Because $g \circ \bar h$ and $\overline{g \circ h}$ are  continuous functions from $\promonad \Sigma$ to a compact Hausdorff space $\balg$, which agree on the injective image of $\monad \Sigma$, they must be  equal by Lemma~\ref{lem:cech-stone}.
% 	\end{pr}
%
%
%
% We are now ready to show that the diagram in~\eqref{eq:gh-diagram} commutes. Recall that this is the diagram:
% 		\begin{align*}
% 	\xymatrix{ \promonad \promonad \Sigma \ar[r]^{\doublebar h} \ar[dr]_{\doublebar{g \circ h}} & A \ar[d]^{g}\\ & B}
% 			\end{align*}
% By unraveling the definitions of $\doublebar h$ and $\doublebar {g \circ h}$, and adding the
% morphism $\promonad g$,  the above diagram becomes
% 				\begin{align*}
% 			\xymatrix{ \promonad \promonad \Sigma \ar[r]^{\promonad \bar h} \ar[dr]_{\promonad \ \overline{g \circ h}}& \promonad A \ar[d]^{\promonad g}\ar[r]^{\overline{\mult_\alg}} & A \ar[d]^{g}\\ & \promonad B \ar[r]^{\overline{\mult_\balg}}  &B} .
% 					\end{align*}
% 					The diagram above commutes because the side to the right of $\promonad g$ is the diagram in Lemma~\ref{lem:chasing-one}, while the diagram to the left of $\promonad g$ is the result of applying the functor $\promonad$ to the diagram in Lemma~\ref{lem:chasing-two}.	 This completes the proof that~\eqref{eq:gh-diagram} commutes, which completes the proof that the multiplication operation $\mult_{\promonad \Sigma}$ satisfies the condition from the statement of the theorem.
